Multi-mode Trajectory Optimization for Impact-aware Manipulation

The transition from free motion to contact is a challenging problem in robotics, in part due to its hybrid nature. Additionally, disregarding the effects of impacts at the motion planning level often results in intractable impulsive contact forces. In this paper, we introduce an impact-aware multi-mode trajectory optimization (TO) method that combines hybrid dynamics and hybrid control in a coherent fashion. A key concept is the incorporation of an explicit contact force transmission model in the TO method. This allows the simultaneous optimization of the contact forces, contact timings, continuous motion trajectories and compliance, while satisfying task constraints. We compare our method against standard compliance control and an impact-agnostic TO method in physical simulations. Further, we experimentally validate the proposed method with a robot manipulator on the task of halting a large-momentum object.

==> figures/tikz/fig_force_66.tex <==
\begin{tikzpicture}
    \begin{axis}[
        xlabel={$t(s)$},
        ylabel={$f(m)$},
        height=2cm,
        ]
        \addplot[
            no markers,
            blue,
        ] table [
            col sep=comma,
            x={time},
            y={force}
        ] {figures/data/force_bag_impact_opt_20kg_066ms_i5_good.dat};
    \end{axis}
\end{tikzpicture}

==> figures/tikz/fig_force_88.tex <==
\begin{tikzpicture}
    \begin{axis}[
        xlabel={$t(s)$},
        ylabel={$f(m)$},
        height=2cm,
        ]
        \addplot[
            no markers,
            blue,
        ] table [
            col sep=comma,
            x={time},
            y={force}
        ] {figures/data/force_bag_impact_opt_20kg_088ms_i10.dat};
    \end{axis}
\end{tikzpicture}
